WiEat: Fine-grained Device-free Eating Monitoring Leveraging Wi-Fi Signals

Eating is a fundamental activity in people's daily life. Studies have shown that many health-related problems such as obesity, diabetes and anemia are closely associated with people's unhealthy eating habits (e.g., skipping meals, eating irregularly and overeating). Traditional eating monitoring solutions relying on self-reports remain an onerous task, while the recent trend requiring users to wear expensive dedicated hardware is still invasive. To overcome these limitations, in this paper, we develop a device-free eating monitoring system using WiFi-enabled devices (e.g., smartphone or laptop). Our system aims to automatically monitor users' eating activities through identifying the fine-grained eating motions and detecting the chewing and swallowing. In particular, our system extracts the fine-grained Channel State Information (CSI) from WiFi signals to distinguish eating from non-eating activities and further recognizing users' detailed eating motions with different utensils (e.g., using a folk, knife, spoon or bare hands). Moreover, the system has the capability of identifying chewing and swallowing through detecting users' minute facial muscle movements based on the derived CSI spectrogram. Such fine-grained eating monitoring results are beneficial to the understanding of the user's eating behaviors and can be used to estimate food intake types and amounts. Extensive experiments with 20 users over 1600-minute eating show that the proposed system can recognize the user's eating motions with up to 95% accuracy and estimate the chewing and swallowing amount with 10% percentage error.

==> text_infocom/implementation.tex <==
\section{Health Assessment}

%Dietary assessment and irregular eating behavior recognition. 
%
%In previous chapter, there are three measurements to achieve the health assessment 1) Food amount estimation represents \textit{how much} you eat; 2) Food type classification represents \textit{what} your eat; 3) Eating behavior tracking represents \textit{when} your eat.
%
%\subsection{Food Amount Estimation}
%To estimate the food amount, researches show that calculating the counts of chews and swallows actions is the crucial method, which reveals the relationship of ingestion activity and total food mass intake. According to the proposed ingestion prediction model by Edward et al.~\cite{sazonov2009toward}, the amount of total food mass intake depends on the total number of chews and swallows during eating period. Since the associated floating mass models for chewing and swallowing are determinate, the average mass per chew and the average mass per swallow subject arranged by individuals' body index range. Therefore, after collecting the accurate counts of the chewing and swallowing for different individuals, we could utilize the specific algorithm called \textit{FACE} to calculate the food intake amount. In that case, referring the standard for calorie level at different groups of food, we use obtained food amount information to calculate the total calories intake for different users. 
%
%To evaluate the healthy states related to food amount information, we define three conditions to describe the user's daily intake calories level: \textbf{Obesity Risk}, \textbf{Overweight Risk} and \textbf{No Weight Gain Risk}. Many studies have showed the majority measurement is the energy gap, the difference of energy intake (EI) and energy expenditure (EE)~\cite{hill2003obesity,wang2012reaching}. Since the diversity of human body index and physiology (e.g., age, sex and physical activity level), the daily calories requirements for different people is variable~\cite{HealthDecember2015}. Therefore, we proposed the \textbf{calories divergence} index to determine the three conditions, represents the difference between the genuine calories intake and recommend calories intake. Scientists points out that 100 Kcal/day~\cite{hill2003obesity} and 382 Kcal/day are the two crucial thresholds for weight gain. In that case, we define \textbf{Obesity Risk} is the \textit{calories divergence} excess 382 Kcal/day; \textbf{Overweight Risk} is the \textit{calories divergence} between 100 Kcal/day to 382 Kcal/day; \textbf{No Weight Gain Risk} is the \textit{calories divergence} lower than 100Kcal/day.
%
%
%\begin{algorithm}[tb]
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}}  % Use Output in the format of Algorithm
%\caption{ FACE: Food Amount Calculation Estimation algorithm }
%\label{alg:Framwork}
%	\begin{algorithmic}[1]
%	\Require
%	The number of chewing counts: $N_{CW}$;
%	The number of swallow counts: $N_{SW}$;
%	Average mass per chewing: $\overline{A}_{CW}$;
%	Average mass per swallow: $\overline{A}_{SW}$;
%	Food category: $i=1,2,3,4,5 ...$;
%	Single food calories per 100 grams: $F_{i}$
%	\Ensure
%	Total mass of chewing activity for food intake measurement: $M_{CW}^{*}$;
%	Total mass of swallow activity for food intake measurement: $M_{SW}^{*}$;
%	Unit food quantity prediction: $Q_i^{*}$;
%	Single food calories intake: $C_{i}^{*}$; 
%	Total calories intake: $C_{total}^{*}$
%			\State $Food Amount Predicition$ = Total Mass of chew and swallow ($N_{CW}$, $N_{SW}$, $\overline{A}_{CW}$, $\overline{A}_{SW}$);
%			\State initial $M_{CW} \gets 0$, $M_{SW} \gets 0$, $Q_i \gets 0$, $C_{i} \gets 0$, $C_{total} \gets 0$
%			\If {\textit{Chew Detect} \textbf{or} \textit{Swallow Detect}}
%				\State $M_{CW} \gets {N_{CW} * \overline{A}_{CW}}$
%				\State $M_{SW} \gets {N_{SW} * \overline{A}_{SW}}$	
%				\State $Q_i \gets (M_{CW} + M_{SW})/2$
%			\EndIf
%			\For { $i=1$; $i++$ }
%				\State $C_{i} \gets  {Q_i * F_i}$
%				\State $C_{total}^{*} \gets  {C_{total} + C_{i}}$
%			\EndFor
%			\State \Return {$Q_i^{*}, C_{total}^{*}$};
%			
%		
%		
%		
%
%	\end{algorithmic}
%\end{algorithm}
%
%\subsection{Food Type Classification}
%
%\subsection{Eating Behavior Tracking}


